Predicting and visualizing psychological attributions with a deep neural network

Judgments about personality based on facial appearance are strong effectors in social decision making, and are known to have impact on areas from presidential elections to jury decisions. Recent work has shown that it is possible to predict perception of memorability, trustworthiness, intelligence and other attributes in human face images. The most successful of these approaches require face images expertly annotated with key facial landmarks. We demonstrate a Convolutional Neural Network (CNN) model that is able to perform the same task without the need for landmark features, thereby greatly increasing efficiency. The model has high accuracy, surpassing human-level performance in some cases. Furthermore, we use a deconvolutional approach to visualize important features for perception of 22 attributes and demonstrate a new method for separately visualizing positive and negative features.

==> table_features.tex <==
\begin{table*}[b]

%\begin{minipage}{\textwidth}
\centering

\caption{
Deconvolved Features. Per attribution, the dataset was binarized into low versus high values (class 0 and 1 respectively) and a deep neural network was trained for classification. Following training, two additional network variants were created retaining only the positive(+) or negative(-) final layer weights. This allows for separate visualization of positive and negative features for each attribution. The images displayed are the averaged deconvolution results over the whole test dataset. For instance, for the attribution gender a pronounced mouth region is common for class 0 (female) while nose and eyebrows are important features for class 1 (male).
}
\label{tab:deconv}

%\vspace*{-0.4cm}
%\changenewpage
%old caption of

\begin{tabular}{
    >{\centering\arraybackslash}p{1.8cm}
    >{\raggedright\arraybackslash}p{1.65cm}
    >{\raggedright\arraybackslash}p{1.65cm}
    >{\raggedright\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{1.8cm}
    >{\raggedright\arraybackslash}p{1.65cm}
    >{\raggedright\arraybackslash}p{1.65cm}
    >{\raggedright\arraybackslash}p{1.65cm}
    }
\toprule
Attribution & Features & Features(-) & Features(+) & Attribution & Features & Features(-) & Features(+)\\
\midrule

~~~age{\newline}(young/old) & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-age)/deconv.png}} &
\parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-age)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-age)/deconv_attr1.png}} &

attractive & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-attractive)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-attractive)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-attractive)/deconv_attr1.png}}\\

calm & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-calm)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-calm)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-calm)/deconv_attr1.png}} &

caring & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-caring)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-caring)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-caring)/deconv_attr1.png}}\\

common & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-common)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-common)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-common)/deconv_attr1.png}} &

confident & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-confident)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-confident)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-confident)/deconv_attr1.png}}\\

egotistic & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-egotistic)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-egotistic)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-egotistic)/deconv_attr1.png}} &

emotional & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-emotional)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-emotional)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-emotional)/deconv_attr1.png}}\\

emotStable & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-emotStable)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-emotStable)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-emotStable)/deconv_attr1.png}} &

familiar & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-familiar)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-familiar)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-familiar)/deconv_attr1.png}}\\

friendly & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-friendly)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-friendly)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-friendly)/deconv_attr1.png}} &
~~gender{\newline}(female/male) & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-gender)/deconv.png}} &
\parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-gender)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-gender)/deconv_attr1.png}}\\

happy & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-happy)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-happy)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-happy)/deconv_attr1.png}} &

intelligent & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-intelligent)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-intelligent)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-intelligent)/deconv_attr1.png}}\\

interesting & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-interesting)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-interesting)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-interesting)/deconv_attr1.png}} &

kind & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-kind)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-kind)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-kind)/deconv_attr1.png}}\\

memorable & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-memorable)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-memorable)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-memorable)/deconv_attr1.png}} &

responsible & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-responsible)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-responsible)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-responsible)/deconv_attr1.png}}\\

sociable & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-sociable)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-sociable)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-sociable)/deconv_attr1.png}} &

trustworthy & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-trustworthy)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-trustworthy)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-trustworthy)/deconv_attr1.png}}\\

typical & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-typical)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-typical)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-typical)/deconv_attr1.png}} &

weird & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-weird)/deconv.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-weird)/deconv_attr0.png}} & \parbox[c]{1em}{\includegraphics[scale=0.98]{images/imgslocal1[bin](meanpixel-weird)/deconv_attr1.png}}\\

\bottomrule
\end{tabular}
%\end{minipage}
\vspace*{-6cm}
\end{table*}
